Adv-OLM: Generating Textual Adversaries via OLM

Deep learning models are susceptible to adversarial examples that have imperceptible perturbations in the original input, resulting in adversarial attacks against these models. Analysis of these attacks on the state of the art transformers in NLP can help improve the robustness of these models against such adversarial inputs. In this paper, we present Adv-OLM, a black-box attack method that adapts the idea of Occlusion and Language Models (OLM) to the current state of the art attack methods. OLM is used to rank words of a sentence, which are later substituted using word replacement strategies. We experimentally show that our approach outperforms other attack methods for several text classification tasks.

==> Adversarial Attack on Text/abstract.tex <==
\begin{abstract}
Deep learning models are susceptible to adversarial examples that have imperceptible perturbations in the original input, resulting in adversarial attacks against these models. Analysis of these attacks on the state of the art transformers in NLP can help improve the robustness of these models against such adversarial inputs. In this paper, we present \textbf{Adv-OLM}, a black-box attack method that adapts the idea of \textbf{O}cclusion and \textbf{L}anguage \textbf{M}odels (OLM) to the current state of the art attack methods. OLM is used to rank words of a sentence, which are later substituted using word replacement strategies. We experimentally show that our approach outperforms other attack methods for several text classification tasks.
\end{abstract}


==> Adversarial Attack on Text/conclusion.tex <==
\section{Conclusion}
\noindent In this work, we present \textbf{Adv-OLM}, a black box attacking method that uses OLM based word ranking strategy, improving the attack performance significantly over previous methods. We also studied how replacing a single variable in a complex system with a new existing method can improve upon the previously existing attack strategies.
For future work, we would like to experiment with other language models in the OLM algorithm. We plan to study the effect of using different transformers for the language model and the target model. 

==> Adversarial Attack on Text/experiments.tex <==
\section{Experiments}
\label{section:experiments}
\noindent We experiment with different benchmark datasets for text classification and entailment: IMDB, AG News, Yelp Polarity and MNLI (details in Appendix \ref{section:dataset}). The statistics of the final dataset are shown in Table \ref{table:dataset}. Test set was randomly choosen stratified set. For evaluating the effectiveness of our proposed approach, we experiment with SOTA text classifiers i.e. transformer based models like BERT \citep{devlin2018bert}, ALBERT \citep{lan2019albert}, RoBERTa \citep{liu2019roberta} and DistilBERT \citep{sanh2019distilbert}.
% We also evaluate our results on a simple BiLSTM model.

We replaced the existing word ranking strategies (i.e. Original (delete)) of previous attack methods: Textfooler \citep{jin2019bert} and BAE-R \citep{garg2020bae} with word rankings generated using OLM and OLM-S while keeping rest of the attack procedure same. The comparison is provided between the attacks generated through original word ranking, and OLM adapted word ranking (including comparison with PWWS attack method \citep{ren2019generating}) in \cref{tab:bertandalbert}, \cref{tab:mnli} and \cref{tab:transformersimdb}. PWWS (Probability Weighted Word Saliency) method considers the word
saliency along with the classification probability. The change in value of the classification probability is used to measure the attack effect of the proposed substitute word, while word saliency shows how well the original word affects the classification. We use the default language model (BERT) employed in the OLM and OLM-S, and %as provided in \citet{harbecke2020considering} 
kept the number of samples generated by the OLM language model as 30 in all the experiments. 

\noindent The following evaluation metrics are used:
\noindent
\begin{itemize}[noitemsep,topsep=-2pt]
    \item \textbf{Attacked Acc.}: Accuracy of the model after attack. Lower the better.
    \item \textbf{Success Rate:} Ratio of number of successful attacks and the total number of attempted attacks\footnote{Note that total number of attempted attacks are not the same as number of input examples i.e., the samples which were originally wrongly classified by the model even before an attack are skipped}. Higher the better.
    \item \textbf{Perturbed Percentage:} Ratio of number of words that were modified by the attack and the total number of words in the input example. Lower the better.
\end{itemize}
We use TextAttack's \citep{morris2020textattack} fine tuned models on these datasets and used it to execute the attacks, including Adv-OLM (Appendix \ref{section:textattack}).

\noindent \textbf{Number of queries in Adv-OLM}:
From equations \ref{eq:OLMlm} and \ref{eq:OLMSsensi}, it is clear that unlike other methods of deletion and \textit{[UNK]} token replacement, which perform only a single query, we need to perform multiple queries. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.48\textwidth]{images/queries.png}
    \caption{Average Number of Queries vs Number of samples in Adv-OLM attack on BERT on IMDB dataset.}
    \label{fig:queries}
\end{figure}
% As we mentioned in \ref{section:experiments}, 
We set the number of samples generated by the OLM language model to 30 for our experiment. In the worst case, we would have all 30 samples of the token as unique, which will query the model 30 times. However, experimentally it was not the case. To study this, we varied the number of samples and evaluated the OLM ranking step's number of queries. In fig \ref{fig:queries}, we plotted the number of queries for OLM averaged over the input samples against the number of samples. We can see that there is not a significant difference in the total number of samples in our case (OLM + Textfooler queries) when compared with PWWS. 


==> Adversarial Attack on Text/intro.tex <==
\section{Introduction}
\noindent In recent times, deep learning models have become pervasive across different domains.
Many of the recent deep models have shown SOTA performance on a variety of NLP tasks \citep{wang2018glue}. 
Consequently, deep models are being deployed in a variety of production systems for real-life applications. 
Hence, it becomes imperative to ensure the reliability and robustness of such models as it might pose a threat to security.

Recent studies have pointed out the vulnerability of deep models to adversarial attacks \citep{goodfellow2014explaining}. Adversarial attack comprises generating adversarial samples by performing small perturbations to the original input, making them imperceptible to humans while fooling the deep learning models to give incorrect predictions. 

% Substantial work is already performed in the field of generating adversarial examples in image and speech domains \citep{szegedy2013intriguing,carlini2018audio}. In computer vision both attack and defense strategies are well-explored \citep{chakraborty2018adversarial}, while generation of adversarial examples for text is challenging because 1) Text is discrete in nature 2) Even small perturbations in text are perceptable to humans 3) Perturbations may change the semantics of a word and a sentence, thus can be easily detected and would heavily affect the model output.

% \citep{jia2017adversarial} are the first to consider generation of textual adversarial examples on deep neural models. Later work followed by applying a variant of gradient based white-box adversarial attacks adopted from images \citep{liang2017deep, sun2018identify,  ebrahimi2017hotflip}. Some more methods craft adversarial samples mainly based on specific rules \citep{gao2018black, li2018textbugger, jin2019bert}. These methods are difficult to guarantee the fluency and semantic preservation in the generated adversarial samples.

% With the advent of number of pretrained models like BERT \citep{devlin2018bert}, RoBERTa \citep{liu2019roberta}, XLNet \citep{yang2019xlnet}, AlBERT \citep{lan2019albert}, the performance for large number of NLP tasks have been pushed further. These models are thus being explored across different use cases. 

% Extensive studies over the robustness of deep learning in Computer Vision has been carried out that perform small perturbations on the original input image \citep{goodfellow2014explaining, kurakin2016adversarial}. These works are mostly focused on using gradient based perturbations. However, 
Adversarial attack on textual data is much more difficult due to the discrete nature of the text. The basic requirement of imperceptibility of perturbation by human judges is much more challenging in a language data setting. Therefore, the adversarial sample needs to be grammatically correct and semantically sound.
Perturbations at word or character level that are perceptible to human judges have been explored in-depth \citep{ebrahimi2017hotflip,belinkov2017synthetic,jia2017adversarial,gao2018black}. Work on defense against misspellings based attacks \citep{pruthi2019combating} and use of optimization algorithms for attacks like genetic algorithm \citep{alzantot2018generating,wang2019natural} and particle swarm optimization \citep{zang2020word} have also been explored. 
% Early works \citep{zhao2017generating} in text adversarial attack focus on variations of gradient-based or otherwise called white-box methods.
% \AM{write a line about what is black box attack} \citet{li2018textbugger} compares both white box and black box type attacks. \AM{what is the purpose of last line, especially since you end the para with it.}
With the rise of pre-trained language models, like BERT \citep{devlin2018bert} and other transformer-based models, generating human imperceptible adversarial examples has become more challenging.  \citet{wallace2019universal},  \citet{jin2019bert}, and \citet{pruthi2019combating} have explored these models from different perspectives.
% \citet{li2020bert} and \citet{garg2020bae} explore some of attack strategies over BERT.
% \AB{Write about white-box and black-box settings.}

Adversarial examples can be generated using black-box, where no knowledge about the model is accessible, and white-box, where information about the technical details of models are known.
Generation of textual adversarial samples in a black-box setting consists of two steps 1) Finding words to replace in a sample (Word Ranking) 2) Replacing the chosen word (Word Replacement). Word Ranking is necessary to ensure that the word that contributes the most to the output prediction is considered as the candidate for replacement in the next step. Other constraints like generating semantically similar adversarial samples, human imperceptibility, and minimal perturbation percentage are also considered. Previous work has obtained word ranking by performing deletion of words 
% (which we refer to as Original (delete) in our paper)
(e.g., BAE-R \citep{garg2020bae}, TextFooler \cite{jin2019bert}),  and replacement of words with \textit{[UNK]} token (e.g., BERT-Attack \citep{li2020bert}) and then ranking the words based on the output logits difference. 

Recently in the model explainability domain, the method of Occlusion and Language Models (OLM) \citep{harbecke2020considering} has been proposed, the authors argue that the data likelihood of the samples obtained after either deleting the token or replacement with \textit{[UNK]} token is very low, which makes these methods unsuitable for determining relevance of the word towards the output probability. The authors propose the use of language models for calculating the relevance of the words in a sentence.
Taking inspiration from OLM, we propose \textbf{Adv-OLM}, a black box attack method, that adapts the idea of OLM (as the Work Ranking Strategy) to find the relevant words to replace.
We empirically show that OLM provides a better set of ranked words compared to the existing word ranking strategies for the generation of adversarial examples.

\noindent We summarize our contributions as follows:
\begin{itemize}[noitemsep,topsep=-2pt]
    \item We propose a new method Adv-OLM, to rank words for generating adversarial examples.
    \item We empirically show that Adv-OLM has a higher success rate and lower perturbation percentage than previous attacking methods.
\end{itemize}

The implementation for the proposed approach is made available at the GitHub repository: \url{https://github.com/vijit-m/Adv-OLM}.
% The implementation of our proposed method will be made available upon acceptance. 





























==> Adversarial Attack on Text/methodology.tex <==
\section{Methodology}
\noindent Adv-OLM uses the idea of Occlusion and Language Models to perform Word Ranking using both OLM and OLM-S methods. %\AM{cite but it is not clear what is OLM or OLM-S is, as said earlier, write it in the intro/relevant work.}
%\AB{Do we need to cite the OLM paper here also, we already did that in the intro part}
OLM uses a language model to sample some candidate instances for a word and then replaces the word. Let $x_{i}$ be a word of the input $x$ and $x_{\backslash i}$ be the incomplete input without this word. Then the OLM relevance score $r$ given the prediction function $f$ and label $y$ is (Here $f_{y}$ is the logit value corresponding to the label $y$.)
%\AM{here you write $f$ but in problem formulation you wrote $F$, make it uniform}
\setlength{\belowdisplayskip}{4pt} \setlength{\belowdisplayshortskip}{4pt}
\setlength{\abovedisplayskip}{4pt} \setlength{\abovedisplayshortskip}{4pt}
\begin{equation} \label{eq:OLMrel}
r_{f,y}(x_{i}) = f_{y}(x_{i}) - f_{y}(x_{\backslash i})
\end{equation}
% \vspace{-5mm}
Here, $f_{y}(x_{\backslash i})$ is not accurately defined and needs to be approximated since $x_{\backslash i}$ is the  incomplete input. A language model $p_{LM}$ generates input by predicting the masked word as $\hat{x_{i}}$ that is as natural as possible for the model and thus approximates to:%\AM{on the right side, why does function $f$ take two arguments? Earlier you define it to take just one argument.}
\begin{equation} \label{eq:OLMlm}
f_{y}(x_{\backslash i}) \approx \sum_{\hat{x_{i}}} p_{LM}(\hat{x_{i}}|x_{\backslash i})f_{y}(x_{\backslash i} \cup \hat{x_{i}}) 
\end{equation}
where, $f_{y}(x_{\backslash i} \cup  \hat{x_{i}}) $ is the prediction of the classification model after the language model's prediction $\hat{x_{i}}$ is added to the incomplete input $x_{\backslash i}$.  

The other method OLM-S calculates the sensitivity of a position in the text and has nothing to do with the word present at that position in the original input. The sensitivity score of OLM-S is calculated
\begin{equation*} \label{eq:OLMSsensi}
\resizebox{.95\hsize}{!}{$
s_{f,y}(x_{i})=\sqrt{\sum_{\hat{x_{i}}} p_{LM}(\hat{x_{i}}|x_{\backslash i})(f_{y}(x_{\backslash i}\cup \hat{x_{i}})-\mu)^{2}} $}
\end{equation*}
where $\mu$ is the mean value from Equation \ref{eq:OLMlm}.
The sensitivity score $s_{f,y}(x_{i})$ is used for word ranking in OLM-S.

After performing the Word Ranking step using the relevance scores generated by OLM and OLM-S, the next step is to replace highly scored words with semantically similar words that form grammatically correct sentences (Word Replacement) such that the output prediction changes. Word replacement strategy is kept similar to existing methods. TextFooler uses Synonym Extraction, POS checking and semantic similarity checking whereas BAE-R uses a Language Model for word replacement. (details in Appendix \ref{section:wordreplacement}).

%---------- Updated Table -----------
\begin{table}[!h]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}}              & \multicolumn{1}{c|}{\textbf{Classes}} & \multicolumn{1}{c|}{\textbf{Train}} & \multicolumn{1}{c|}{\textbf{Test}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg. Length
% \footnote{Average Sequence Length of Test Set} 
\end{tabular}}} \\ \hline \hline
\multicolumn{5}{|c|}{\textbf{Classification}} \\ \hline 
IMDB & 2 & 25K & 500 & 245.12                   
\\ \hline
Yelp & 2 & 560K & 500 & 132.33                  
\\ \hline
\begin{tabular}[c]{@{}l@{}}AG's News\end{tabular} & 4 & 120K & 500 & 40.41                          \\ \hline
\multicolumn{5}{|c|}{\textbf{Natural Language Inference}}       
\\ \hline
MNLI & 3 & 433K & 500 & 29.72                   
\\ \hline
\end{tabular}
}
\caption{Statistic of Datasets. Avg. Length is the average number of words in the test set.}
\label{table:dataset}
\end{table}

%--------------- AG and Yelp -------------------

\begin{table*}[t]\small
\renewcommand{\arraystretch}{1.5}
% Default value: 1
\centering

% \hspace*{-3em}
\setlength\tabcolsep{3.5pt}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|ccc|c|ccc|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Word Ranking}} & \multicolumn{4}{c|}{\textbf{BERT}} & \multicolumn{4}{c|}{\textbf{ALBERT}}              \\ \cline{4-11} &  &  & 
\textbf{Original Acc.}  & \multicolumn{1}{c|}{\textbf{Attacked Acc.}} & \multicolumn{1}{c|}{\textbf{Success Rate}} & \multicolumn{1}{c|}{\textbf{Perturbed \%}} & \textbf{Original Acc.}  & \multicolumn{1}{c|}{\textbf{Attacked Acc.}} & \multicolumn{1}{c|}{\textbf{Success Rate}} & \multicolumn{1}{c|}{\textbf{Perturbed \%}} \\ \hline \hline
\multirow{7}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}AG's\\ News\end{tabular}}} & 

\multirow{3}{*}{BAE-R} & OLM  & \multirow{7}{*}{93.8\%} & \multicolumn{1}{c|}{\textbf{78\%}}  & \multicolumn{1}{c|}{\textbf{16.84\%}}  & \multicolumn{1}{c|}{6.72\%}   & \multirow{7}{*}{94.4\%} & \multicolumn{1}{c|}{\textbf{79.2\%}}  & \multicolumn{1}{c|}{\textbf{16.1\%}} & \multicolumn{1}{c|}{8.37\%} \\
 &   & OLM-S   &    & \multicolumn{1}{c|}{79\%}  & \multicolumn{1}{c|}{15.78\%}  & \multicolumn{1}{c|}{\textbf{6.35\%}}  &  & \multicolumn{1}{c|}{82.4\%}  & \multicolumn{1}{c|}{12.71\%} & \multicolumn{1}{c|}{\textbf{6.9\%}} \\
 &  & Original (delete) &    & \multicolumn{1}{c|}{78.8\%}   & \multicolumn{1}{c|}{15.99\%}     & \multicolumn{1}{c|}{6.42\%}  &  & \multicolumn{1}{c|}{79.4\%}  & \multicolumn{1}{c|}{15.89\%}  & \multicolumn{1}{c|}{7.67\%}  \\ 
 \cline{2-3} \cline{5-7} \cline{9-11} 
 
 & \multirow{3}{*}{TextFooler} & OLM  &  & \multicolumn{1}{c|}{\textbf{19.2\%}}    &    \multicolumn{1}{c|}{\textbf{79.53\%}}     & \multicolumn{1}{c|}{23.52\%}  &    & \multicolumn{1}{c|}{20.4\%} & \multicolumn{1}{c|}{78.39\%}  & \multicolumn{1}{c|}{21.24\%} \\   
 &  & OLM-S  &  & \multicolumn{1}{c|}{21.4\%}  & \multicolumn{1}{c|}{77.19\%} & \multicolumn{1}{c|}{\textbf{20.96\%}}  &   &\multicolumn{1}{c|}{\textbf{20.2\%}}  & \multicolumn{1}{c|}{\textbf{78.6\%}} & \multicolumn{1}{c|}{\textbf{20.18\%}} \\ 
 &  & Original (delete)  &   & \multicolumn{1}{c|}{21.4\%}  & \multicolumn{1}{c|}{77.19\%} & \multicolumn{1}{c|}{23.19\%}   & & \multicolumn{1}{c|}{22.0\%} & \multicolumn{1}{c|}{76.69\%}  & \multicolumn{1}{c|}{21.15\%} \\ 
 \cline{2-3} \cline{5-7} \cline{9-11}
 & PWWS  & - &  & \multicolumn{1}{c|}{44.8\%}  & \multicolumn{1}{c|}{52.24\%} & \multicolumn{1}{c|}{16.21\%}    &    & \multicolumn{1}{c|}{36.8\%}  & \multicolumn{1}{c|}{61.02\%}  & \multicolumn{1}{c|}{14.8\%}  \\ \hline
 
\multirow{7}{*}{\textbf{Yelp}} & \multirow{3}{*}{BAE-R} 
& OLM  & \multirow{7}{*}{97.2\%} & \multicolumn{1}{c|}{\textbf{38.4\%}} & \multicolumn{1}{c|}{\textbf{60.49\%}} & \multicolumn{1}{c|}{\textbf{6.45\%}} & \multirow{7}{*}{97.4\%} & \multicolumn{1}{c|}{41.4\%} & \multicolumn{1}{c|}{57.49\%} & \multicolumn{1}{c|}{7.07\%} \\ 
&  & OLM-S  & & \multicolumn{1}{c|}{55.2\%}  & \multicolumn{1}{c|}{43.21\%}  & \multicolumn{1}{c|}{10.36\%}  &   & \multicolumn{1}{c|}{39.6\%}  & \multicolumn{1}{c|}{59.34\%} & \multicolumn{1}{c|}{7.11\%} \\ 
&  & Original (delete) &  & \multicolumn{1}{c|}{41.6\%}  & \multicolumn{1}{c|}{57.20\%}  & \multicolumn{1}{c|}{7.28\%}   &   & \multicolumn{1}{c|}{35.0\%} & \multicolumn{1}{c|}{64.07\%}  & \multicolumn{1}{c|}{6.49\%} \\ \cline{2-3} \cline{5-7} \cline{9-11} 
& \multirow{3}{*}{TextFooler}      
& OLM &  & \multicolumn{1}{c|}{\textbf{5.2\%}} & \multicolumn{1}{c|}{\textbf{94.65\%}} & \multicolumn{1}{c|}{\textbf{9.10\%}}  &   & \multicolumn{1}{c|}{\textbf{2.6\%}}         & \multicolumn{1}{c|}{\textbf{97.33\%}}  & \multicolumn{1}{c|}{10.17\%}  \\ 
&  & OLM-S   &   & \multicolumn{1}{c|}{7.8\%}   & \multicolumn{1}{c|}{91.98\%}  & \multicolumn{1}{c|}{13.31\%}  &   & \multicolumn{1}{c|}{2.8\%}   & \multicolumn{1}{c|}{97.13\%} & \multicolumn{1}{c|}{10.13\%} \\
&  & Original (delete)   &   & \multicolumn{1}{c|}{6.6\%} & \multicolumn{1}{c|}{93.21\%}   & \multicolumn{1}{c|}{9.95\%}  & & \multicolumn{1}{c|}{3.8\%}  & \multicolumn{1}{c|}{96.1\%}  & \multicolumn{1}{c|}{9.57\%} \\ \cline{2-3} \cline{5-7} \cline{9-11}
& PWWS  & -   &    & \multicolumn{1}{c|}{6.2\%}  & \multicolumn{1}{c|}{93.62\%}  & \multicolumn{1}{c|}{6.9\%}   &   & \multicolumn{1}{c|}{3.8\%}   & \multicolumn{1}{c|}{96.1\%}   & \multicolumn{1}{c|}{6.82\%} \\ \hline
\end{tabular}
}
\caption{Comparison between word ranking strategies on AG's News and Yelp for fine-tuned BERT and ALBERT. Our method Adv-OLM has OLM (or OLM-S) as the word ranking strategy.}
\label{tab:bertandalbert}

\end{table*}

%------------------- MNLI ------------------------------

\begin{table*}[h!]\small
\renewcommand{\arraystretch}{1.5} % Default value: 1
\centering
\setlength\tabcolsep{3.5pt}
\resizebox{1.3\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Dataset\end{tabular}} & 
\textbf{Method} & 
\textbf{\begin{tabular}[c]{@{}c@{}}Word Ranking\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Original Acc.\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Attacked Acc.\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Success Rate\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Perturbed \%\end{tabular}}  
\\ \hline \hline
\multirow{7}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}MNLI\end{tabular}}} &
\multirow{3}{*}{BAE-R} & 
OLM & \multirow{7}{*}{84.6\%} & 20.6\% & 75.65\% & 7.82\%   
\\ 
% \cline{3-3} \cline{5-7} 
& & 

OLM-S & & 20.8\% & 75.41\% & 8.22\%
\\ 
% \cline{3-3} \cline{5-7}
& & 

\begin{tabular}[c]{@{}c@{}}Original (delete)\end{tabular} & & 
14.0\% & 83.45\% & 6.4\%                                             \\ \cline{2-3} \cline{5-7} & 

\multirow{3}{*}{TextFooler} & OLM & & 
\textbf{6.6\%} & \textbf{92.2\%} & 8.29\%                           \\
% \cline{3-3} \cline{5-7}
& & 

OLM-S & & 7.0\% & 91.73\% & 8.59\%
\\ 
% \cline{3-3} \cline{5-7} 
& & 

\begin{tabular}[c]{@{}c@{}}Original (delete)\end{tabular} & & 
6.8\% & 91.96\% & 6.98\%
\\ \cline{2-3} \cline{5-7} & 

PWWS & - & & 3.2\% & 96.22\% & 6.62\%                               \\ \hline

\end{tabular}
}
\caption{Comparsion between previous methods and Adv-OLM on MNLI fine-tuned BERT. Our method Adv-OLM has OLM (or OLM-S) as the word ranking strategy.}
\label{tab:mnli}
\end{table*}


% ---------------- IMDB across models -----------

\begin{table*}[h!]\small
\renewcommand{\arraystretch}{1.5} % Default value: 1
\centering
\setlength\tabcolsep{5pt}
\resizebox{1.4\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Model} &
\textbf{Method} & 
\textbf{
\begin{tabular}[c]{@{}c@{}}Word Ranking\end{tabular}} &
\textbf{Original Acc.}  & 
\textbf{Attacked Acc.} & 
\textbf{Success Rate} & 
\textbf{Perturbed \%} 
\\ \hline \hline

\multirow{7}{*}{\textbf{BERT}} & 
\multirow{3}{*}{BAE-R} & OLM & 
\multirow{7}{*}{92.0\%} & 38.8\% & 57.83\% & 2.79\%
\\ 
% \cline{3-3} \cline{5-7}
& & 

OLM-S & & \textbf{33.2\%} & \textbf{63.91\%} & \textbf{2.33\%} 
\\ 
% \cline{3-3} \cline{5-7} 
& & 

Original (delete) & & 42.6\% & 53.70\% & 2.92\%
\\ \cline{2-3} \cline{5-7} & 

\multirow{3}{*}{Textfooler} & 
OLM & & 29.8\% & 67.61\% & 4.52\%
\\
% \cline{3-3} \cline{5-7} 
& & 

OLM-S & & \textbf{26.4\%} & \textbf{71.3\%} & \textbf{3.16\%}
\\ 
% \cline{3-3} \cline{5-7}
& & 

Original (delete) &  & 31.8\% & 65.43\% & 5.26\%
\\ \cline{2-3} \cline{5-7} & 

PWWS & \_ & & 28.2\% & 69.35\% & 2.92\% \\ \hline

\multirow{7}{*}{\textbf{ALBERT}} &
\multirow{3}{*}{BAE-R} & 
OLM & \multirow{7}{*}{92.8\%} & 27.4\% & 70.47\% & 3.58\% 
\\ 
% \cline{3-3} \cline{5-7} 
& & 

OLM-S & & \textbf{23.2\%}  & \textbf{75.0\%} & \textbf{3.4\%}
\\ 
% \cline{3-3} \cline{5-7}
& & 

Original (delete) & & 26.8\% & 71.12\% & 3.48\%
\\ 
\cline{2-3} \cline{5-7} 
& 

\multirow{3}{*}{Textfooler} & 
OLM & & \textbf{1.4\%} & \textbf{98.49\%} & 6.65\%
\\ 
% \cline{3-3} \cline{5-7}
& & 

OLM-S &  & \textbf{1.4\%} & \textbf{98.49\%} & \textbf{5.39\%} 
\\
% \cline{3-3} \cline{5-7} 
& & 

Original (delete) & & 2.4\%  & 97.41\% & 6.57\%
\\ \cline{2-3} \cline{5-7}  &

PWWS & \_ & & 3.8\% & 95.91\% & 3.76\% \\ \hline

\multirow{7}{*}{\textbf{RoBERTa}} & 
\multirow{3}{*}{BAE-R} & 
OLM & \multirow{7}{*}{94.2\%} & 29.4\% & 68.79\% & 4.08\%  
\\
% \cline{3-3} \cline{5-7}
& & 

OLM-S &  & \textbf{28.0\%}  & \textbf{70.28\%} & \textbf{3.57\%}
\\ 
% \cline{3-3} \cline{5-7}
& & 

Original (delete) &  & 29.4\%  & 68.79\% & 3.9\% \\ 
\cline{2-3} \cline{5-7} &

\multirow{3}{*}{Textfooler} & 
OLM  &  & \textbf{0.0\%}    & \textbf{100\%} & 7.62\% 
\\ 
% \cline{3-3} \cline{5-7}
& & 

OLM-S & & 0.2\% & 99.79\% & \textbf{6.43\%} 
\\
% \cline{3-3} \cline{5-7}
& & 

Original (delete) & & 0.2\% & 99.79\% & 6.89\%
\\
% \cline{2-3} \cline{5-7} 
& 

PWWS & \_ & & 0.4\% & 99.58\% & 5.38\%  
\\ \hline

\multirow{7}{*}{\textbf{DistilBERT}} & \multirow{3}{*}{BAE-R} & 
OLM & 
\multirow{7}{*}{91.8\%} & 22.6\% & 75.38\% & 3.29\%  
\\ 
% \cline{3-3} \cline{5-7} 
& & 

OLM-S & & 21.6\% & 76.47\% & \textbf{2.93\%} 
\\
% \cline{3-3} \cline{5-7} 
& & 

Original (delete) & & 21.6\% & 76.47\% & 3.34\% 
\\ \cline{2-3} \cline{5-7} & 

\multirow{3}{*}{Textfooler} & 
OLM & & 0.2\% & 99.78\% & 4.03\% 
\\ 
% \cline{3-3} \cline{5-7}
& & 

OLM-S & & 0.2\% & 99.78\% & \textbf{3.55\%} 
\\ 
% \cline{3-3} \cline{5-7} 
& & 

Original (delete) &  & 0.2\%  & 99.78\% & 4.44\% 
\\ \cline{2-3} \cline{5-7} & 

PWWS & \_ & & 0.6\% & 99.35\% & 3.0\%
\\ \hline

\multirow{7}{*}{\textbf{BiLSTM}} & 
\multirow{3}{*}{BAE-R} & 
OLM & \multirow{7}{*}{83.8\%} & 10.8\% & 87.11\% & 2.78\% 
\\ 
% \cline{3-3} \cline{5-7}
& & 

OLM-S & & 10.4\% & 87.59\% & 2.71\% 
\\ 
% \cline{3-3} \cline{5-7} 
& & 

Original (delete) & & 8.6\% & 89.74\% & 2.52\% 
\\ \cline{2-3} \cline{5-7} & 

\multirow{3}{*}{Textfooler} & OLM & & 0\% & 100\% & 2.38\% 
\\ 
% \cline{3-3} \cline{5-7}
& & 

OLM-S &  & 0\% & 100\%  & 2.41\%
\\ 
% \cline{3-3} \cline{5-7} 
& & 

Original (delete) & & 0\%  & 100\% & 1.95\% 
\\ \cline{2-3} \cline{5-7} & 

PWWS & \_ & & 0\% & 100\% & 1.63\% \\ \hline

\end{tabular}
}
\caption{Comparison between previous methods and Adv-OLM for IMDB dataset across different models. Our method Adv-OLM has OLM (or OLM-S) as the word ranking strategy.}
\label{tab:transformersimdb}
\end{table*}



==> Adversarial Attack on Text/problem.tex <==
\section{Problem Formulation}
\noindent We are given a corpus consisting of $n$ input samples, $\mathbb{X} = \{x_1,\ldots , x_n\}$ with corresponding labels $\mathbb{Y} = \{y_1, \ldots , y_n\}$ and a trained classification model $f (f : \mathbb{X} \rightarrow \mathbb{Y})$ that maps an input samples to its correct label. We assume a black-box setting where the attacker can only query the classifier for output label probabilities for the given input. For an input sample $x \in \mathbb{X}$, the task is to construct an adversarial sample $x^{\prime}$ such that, $f(x) = y, \quad f(x^{\prime}) = y^{\prime}$ with $\quad y \neq y^{\prime}$, and $Similarity(x^{\prime},x) \geq \epsilon$. 
Here, $Similarity: \mathbb{X}\times\mathbb{X}\rightarrow(0,1)$ can be both the semantic and syntactic similarity function, and $\epsilon$ is the minimum similarity threshold. Ideally, the amount of perturbation should be minimized. 
The first step is to rank the words of the sample $x$.
% Then based on the ranking, starting from the most important word, the word is replaced by some candidate word which keeps the perturbed sample $x^{'}$ semantically and grammatically sound and also changes the output prediction.
Based on the ranking, starting from the most important word, the word is replaced by some candidate word that keeps the perturbed sample $x^{\prime}$ semantically similar and grammatically sound but changes the output prediction.

% % --------- textfooler imdb + olm example -----------------

\begin{figure*}[!ht]
\centering
\begin{subfigure}{\textwidth}
  \includegraphics[width=1\linewidth]{images/textfooler_imdb_example.png}
  \caption{TextFooler Attack on fine-tuned BERT on IMDB data sample. $[\textcolor{red}{Negative (100\%)} \rightarrow \textcolor{green}{Positive (59\%)}]$
  }
  \label{fig:textfooler_imdb}
\end{subfigure}

\begin{subfigure}{\textwidth}
  \includegraphics[width=1\linewidth]{images/textfooler_olm_imdb.png}
  \caption{Adv-OLM Attack on fine-tuned BERT on IMDB data sample.
    $[\textcolor{red}{Negative (100\%)} \rightarrow \textcolor{green}{Positive( 95\%)}]$
    }
    \label{fig:textfooler_olm_imdb}
\end{subfigure}
\caption{Qualitative Examples of TextFooler and Adv-OLM on BERT classifier (\textcolor{red}{Red} words are replaced by \textcolor{green}{Green} words while changing the output prediction probability.)}
\label{fig:textfooler_olm_example}
\end{figure*}

==> Adversarial Attack on Text/relatedwork.tex <==
% \section{Related Work}
% Extensive studies over the robustness of deep learning models on the continuous data have been carried out that use small perturbations to the original inputs \citep{goodfellow2014explaining}, \citep{kurakin2016adversarial}. These works were mostly focused on computer vision tasks and typically use gradient based perturbations. However, adversarial attacks on textual data is much more difficult due to the discrete nature of text. The basic requirement of the imperceptibility of the perturbation by human judges is much more challenging in such discrete data. Another condition that is needed in case of text is that the adversarial example should be gramatically correct and semantically consistent with the original inputs. This is why, to ensure the robustness and reliability of neural networks in linguistics domain, it is necessary to explore the attack strategies.



% Early works in text adversarial attack focus on variations of gradient-based or otherwise called white-box methods. For example, \citep{zhao2017generating} transform input data into a latent representation by the use of Generative Adversarial Networks (GANs). \citep{li2018textbugger} compares both white box and black box type attacks.

% Perturbations on word or character level, have been explored in \citep{alzantot2018generating}, \citep{ebrahimi2017hotflip}, \citep{belinkov2017synthetic}. \citep{jia2017adversarial}, \citep{gao2018black}, which are perceptible to human judges. Works on defense against misspellings based attacks have also been done \citep{pruthi2019combating}. The use of optimization algorithms for attacks like genetic algorithm \citep{alzantot2018generating}, \citep{wang2019natural} and particle swarm optimization \citep{zang2020word} have also been explored.

% With the rise of pre-trained language models, like BERT \citep{devlin2018bert}, RoBERTa \citep{liu2019roberta} and XLNet \citep{yang2019xlnet}, the difficulty of generating human imperceptible adversarial examples has increased a lot. Exploration of these models from different perspectives \citep{wallace2019universal}, \citep{jin2019bert} \citep{pruthi2019combating} have been performed. \citep{li2020bert} and \cite{garg2020bae} explore some of attack strategies over BERT.

% In general, most of the attack strategies in the black-box setting include word-ranking as the first step using the output probabilities of the model. For this task, several strategies have been explored \citep{ren2019generating}, \citep{jin2019bert}.

% Although most of the attacks have been carried out on classification tasks like sentiment analysis and Natural Language Inference, there have also been works on QA tasks like \citep{wang2018robust} and \citep{jia2017adversarial}.

% \section{Motivation behind OLM paper}
% For explaining a black box model, token level attributions play a significant role. The method of occlusion used in past papers usually either delete the token or replace the token with an \textit{\textless UNK \textgreater} token to measure the importance of that token.
% \begin{equation}
% r_{f,c}(x_{i}) = f_{c}(x_{i}) - f_{c}(x_{\backslash i})
% \end{equation}
% Therefore in the above equation $f_{c}(x_{\backslash i})$ where $x_{\backslash i}$ is the input with perturbation of token $x_{i}$, is not reliable.

% In the paper \citep{harbecke2020considering}, the authors argue that the likelihood of such an input (with either deletion or unknown token replacement method) is usually negative and the predictions of the model over these inputs is not meaningful. 

% To generate meaningful replacements of tokens they use the capabilities of the BERT language model as it generates input that is as natural as possible for the model. And so they approximate the value of $f_{c}(x_{\backslash i})$ by the following equation.
% \begin{equation}
% f_{c}(x_{\backslash i}) \approx \sum_{x_{i}} p_{LM}(\hat{x_{i}}|x_{\backslash i})f_{c}(x_{\backslash i},\hat{x_{i}})
% \end{equation}
% The OLM-S is basically the variance whereas OLM is the wieghted average of the Language Model's predictions. Note that OLM-S is independent of the original token at that position.
% \begin{equation}
% s_{f,c}(x_{i})=\sqrt{\sum_{x_{i}} p_{LM}(\hat{x_{i}}|x_{\backslash i})(f_{c}(x_{\backslash i},\hat{x_{i}}) - \mu)^{2}}
% \end{equation}
% The word-level or token-level ranking is important in the task of adversarial attacks. Rather than perturbing the input instance randomly, perturbing the input instance at the location of a token that is very important for prediction is a viable strategy. Although the fact that OLM based method samples replacement candidates in the approximation of $f_{c}(x_{\backslash i})$, and thus increasing the number of queries is a downside, we will ignore it for our further experiments.

% Also, as far as we know, no study has been conducted that compares the attacks based on the point of view of different word ranking strategies. This will be a novelty from our side.








==> Adversarial Attack on Text/results.tex <==
\section{Results and Analysis}
\noindent Results are shown in Tables \ref{tab:bertandalbert}, \ref{tab:mnli} and \ref{tab:transformersimdb}. Table \ref{tab:bertandalbert} provides the results on AG News and Yelp datasets on fine-tuned BERT and ALBERT model. Our method performs better on both datasets by increasing the success rate by about 1-3\% than the previous methods and also decreasing the perturbation percentage.
Table \ref{tab:mnli} gives the results of attacking a fine-tuned BERT on MNLI.  Although we did not perform better than original BAE-R, we were still able to outperform TextFooler. Due to the unavailability of MNLI fine-tuned ALBERT model in TextAttack, we did not perform an attack on ALBERT. It can also be seen from Table \ref{tab:bertandalbert} that the perturbation percentage for AG's News exceed more than 20\%, which seems to be a perceptible change, but since the average length of the article is only 40.41, making the space for finding relevant words less, the perturbation percentage becomes very high.

To compare attacks across different transformer-based models, we evaluate the performance of Adv-OLM on IMDB dataset. Table \ref{tab:transformersimdb} provides the results of different attack methods on BERT, ALBERT, RoBERTa, DistilBERT and BiLSTM.
% and BiLSTM models. 
Adv-OLM was able to outperform previous attack methods on BERT, ALBERT, RoBERTa by increasing the success rate up to 10\% for BAE-R and up to 6\% for TextFooler. Perturbation percentage was also reduced by 1-2\%. On DistilBERT, Adv-OLM showed no change in the success rate, but the perturbation percentage was lowered slightly.
We also performed an attack on a non-transformer based BiLSTM model which did not show any improvements in the success rate. For BAE-R, it even showed a decrease in the success rate for Adv-OLM. One possible reason for this might be that in both OLM and OLM-S word sampling is performed using a transformer-based BERT language model. We also have qualitative results on IMDB dataset (Figure \ref{fig:textfooler_imdb}, \ref{fig:textfooler_olm_imdb}  in Appendix).

Experimentally it was observed that better words were ranked when OLM/OLM-S was used as the Word Ranking strategy (Figure \ref{fig:textfooler_olm_imdb}). 
% We also perform an analysis of the average number of queries and the number of samples used in OLM language model. It is observed that there is a linear increase in the number of queries on increasing the number of samples for the language model, although textfooler queries with OLM word rankings show a decreasing trend, the overall number of queries for Adv-OLM (which combined both language model generated and textfooler generated queries) increase with increasing average number of samples (c.f. Appendix \ref{section:analysis_num_queries}).
When comparing with the original methods, Adv-OLM has more number of queries, which is due to the fact that for word rankings, OLM/OLM-S queries the model a  number of times, thus increasing the overall queries. However, the difference in the number of Adv-OLM queries with the existing attacking methods is not very significant since the model is queried only for unique words from the samples generated from the language model.
